Collaborating in a competitive world: Heterogeneous Multi-Agent Decision Making in Symbiotic Supply Chain Environments

Supply networks require collaboration in a competitive environment. To achieve this, nodes in the network often form symbiotic relationships as they can be adversely effected by the closure of companies in the network, especially where products are niche. However, balancing support for other nodes in the network against profit is challenging. Agents are increasingly being explored to define optimal strategies in these complex networks. However, to date much of the literature focuses on homogeneous agents where a single policy controls all of the nodes. This isn't realistic for many supply chains as this level of information sharing would require an exceptionally close relationship. This paper therefore compares the behaviour of this type of agent to a heterogeneous structure, where the agents each have separate polices, to solve the product ordering and pricing problem. An approach to reward sharing is developed that doesn't require sharing profit. The homogenous and heterogeneous agents exhibit different behaviours, with the homogenous retailer retaining high inventories and witnessing high levels of backlog while the heterogeneous agents show a typical order strategy. This leads to the heterogeneous agents mitigating the bullwhip effect whereas the homogenous agents do not. In the high demand environment, the agent architecture dominates performance with the Soft Actor-Critic (SAC) agents outperforming the Proximal Policy Optimisation (PPO) agents. Here, the factory controls the supply chain. In the low demand environment the homogenous agents outperform the heterogeneous agents. Control of the supply chain shifts significantly, with the retailer outperforming the factory by a significant margin.

==> ResultPea.tex <==
\section{Comparison of homogeneous and heterogeneous agents in the low demand environment}

A numerical analysis is conducted to compare the performance of homogeneous and heterogeneous agents on an environment with a lower demand to see how the agent architectures affect the order strategies. First, the behavior of the SAC and PPO agents is assessed on the baseline environment, followed by efforts to improve cooperation through reward sharing without sharing profit.

\subsection{Comparisons of the homogeneous and heterogeneous agents on the low demand baseline environment}
Agents are much less profitable in a low demand scenario compared to a high demand scenario. Figure \ref{fig:episode-reward-low} shows that in the low demand example the heterogeneous agents receives lower rewards compared to the homogeneous agents, with the SAC agent able to generate 128.8 and the PPO generating 199.9 while the homogeneous SAC agent generates 2384.8 and the homogeneous PPO generating a lower reward of 1505.  

\begin{figure*}[!htbp]
    \centering
 \begin{subfigure}[!htbp]{0.485\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/SEnv1PS-.png}
\subcaption{Homogeneous agent .}
\end{subfigure}
\begin{subfigure}[!htbp]{0.485\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/Env1PS-.png}
\subcaption{Heterogeneous agent.}
\end{subfigure}
\caption{Homogeneous and Heterogeneous agent's performance in the low demand environment. The shaded area depicts the standard deviation of the multi-agent's performance for independent experiments using 5 different seeds.}
\label{fig:episode-reward-low}
\end{figure*}

%18th Dec

Figure \ref{fig:factory-retailer-reward-low1} demonstrates that for both the PPO and SAC algorithms the  factory profit ends up lower than the retailer profit. For the PPO agent the retailer profit is 164.6 and the factory is 63.2 while for the SAC the Retailer is 171.52 and the factory generates a negative reward of -28.9. In the SAC agent, the retailer immediately finds a strategy that works well and stays at a similar reward with the factory agent iterating towards a maximum reward. However, in these scenarios almost all of the agents are able to find a strategy to make a profit. 


\begin{figure*}[!htbp]
    \centering
        \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2SACEnv1.png}
  \subcaption{SAC}    \label{fig:episode}
  \end{subfigure}
    \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2PPOEnv1.png}
  \subcaption{PPO}
\label{fig:episode}
  \end{subfigure}
\caption{Low Demand heterogeneous agent's retailer and factory performance where the shaded area depicts the standard deviation of the independent experiments using 5 different seeds.}
\label{fig:factory-retailer-reward-low1}
\end{figure*}

In the low demand environment it is easier for the agent to avoid backlog and stockout. The ordering strategies show some similarities to the high demand strategy but in this scenario it is easier for the agent to control the inventory. The homogeneous retailer agent keeps the stock at a high level, similar to in the high demand scenario, demonstrated in Figure \ref{fig:stockout-backlog-high2-homo}. This incurs a large number of backlog penalties but never incurs a stockout. The factory agent is able to respond with a regular
% buying
inventory strategy% approach
, 
buying 9 or 10 items every few cycles and waiting for this stock to get used up.
%%%%%3112
The factory in this environment, the overall inventory level remains low with a mean of 1.84. 
This incurs no stockout or backlog penalties. 

\begin{figure*}[!htbp]
    % \begin{subfigure}[b]{0.51\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth, height=4.1cm]{figures/SP1+BS.png} % Adjust the width to fit inside the subfigure
    %     \caption{Homogeneous PPO.}
    % \end{subfigure}
    % \ContinuedFloat
    % \begin{subfigure}[b]{0.51\linewidth}
    %     \centering
        \includegraphics[width=\linewidth, height=6.6cm]{figures/SSBSENV1R.png} % Adjust the width to fit inside the subfigure
        % \caption{Homogeneous agent.}
    % \end{subfigure}
     \caption{Homogeneous SAC agent actions and resulting backlog and stockouts in the low demand scenario. The inventory of the factory is 1.84 while the inventory of the retailer is 19.0. These methods have been proven to reduce the risk of stock-outs and backlogs in the supply chain by learning effective inventory strategies. }
     \label{fig:stockout-backlog-high2-homo}
\end{figure*}




In the heterogeneous agent then there is a less structured buying profile, with the retailer agent buying to the maximum stock level and then letting this reduce to empty, shown in Figure \ref{fig:stockout-backlog-low1-Hetero}. The factory agent also keeps a lower stock level 1.84 than in the homogeneous agent 21. In this case the agent tends to immediately recover it's stock level to the maximum as soon as possible, never allowing the stock to stay at a low level.  

\begin{figure*}[!htbp]
    % \begin{subfigure}[b]{0.71\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=6.4cm]{figures/mS1sb-.png} % Adjust the width to fit inside the subfigure  in Env1
    %     \caption{Heterogeneous PPO.}
    % \end{subfigure}
    % \ContinuedFloat
    % \begin{subfigure}[b]{0.51\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth, height=4.1cm]{figures/ms1sbh.png} % Adjust the width to fit inside the subfigure in Env1(High Demand)
    %     \caption{Heterogeneous SAC.}
    % \end{subfigure}
     \caption{Heterogeneous SAC agent actions and resulting backlog and stockouts in the low demand scenario. The inventory of the factory is 21 while the inventory of the retailer is 8. These methods have been proven to reduce the risk of stock-outs and backlogs in the supply chain by learning effective inventory strategies.}
     \label{fig:stockout-backlog-low1-Hetero}
\end{figure*}

Similarly to the high demand scenario, the price for the different agents shows a clear relation to the performance. In this case the homogenous agents charge the higher price, with the SAC agent charging 56.93 and the PPO agent charging 52.67. This is substantially higher than the heterogeneous agents, that charge the lowest amount with the heterogeneous PPO agent charging 36.88 and the heterogeneous agent charging 30.82. In the heterogenous cases, for both the PPO and the SAC agents, the variation across the range of different potential prices is high, there is no consistency with the agent sometimes selecting values in the 50-60 range but also selecting in the 0-10 range. However, in the homogenous PPO agent the 

\begin{figure*}[!htbp]
    % \begin{subfigure}[b]{0.71\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=6.4cm]{figures/Low Demand Price11.png} % Adjust the width to fit inside the subfigure  in Env1
    %     \caption{Heterogeneous PPO.}
    % \end{subfigure}
    % \ContinuedFloat
    % \begin{subfigure}[b]{0.51\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth, height=4.1cm]{figures/ms1sbh.png} % Adjust the width to fit inside the subfigure in Env1(High Demand)
    %     \caption{Heterogeneous SAC.}
    % \end{subfigure}
     \caption{Comparison of cost across the different agents in the low demand environment}
     \label{fig:Low-Demand-Price}
\end{figure*}



\subsection{Reward shaping to increase collaboration between agents in the low demand environment}
\label{Reward shaping low}
The homogeneous agent also outperforms the heterogeneous agents with reward shaping. 
The homogeneous agents also have a lower percentage variation in performance with the 5 simulations varying by 1505.0 and 2384.8 while the variation in the heterogeneous agent is higher, 128.8 and 199.9. 
For the PeaRSO reward structure the heterogeneous SAC agent has a maximum reward of 200.85 and the PPO agent has 174.83 while the homogeneous SAC agent reaches rewards of 2391.6 and the PPO agent reaches 1374.8. This is similar in the PeaFSO reward structure the heterogeneous SAC agent has a maximum reward of 161.2 and the PPO agent has 212.6 while the homogeneous SAC agent reaches rewards of 2387.9 and the PPO agent reaches 1356.3. 
%%%%++3012
In the Colla reward structure the heterogeneous SAC agent has a maximum reward of 224.1 and the PPO agent has  224.0 while the homogeneous SAC agent reaches rewards of 2392.2 and the PPO agent reaches 1229.0.
The rewards for the PeaRSO environment are a little higher for the homogeneous agent while for the heterogeneous agents the PeaFSO reward shaping the PPO agent has a higher reward and the SAC has a higher reward with the PeaRSO. 
%%%%++3012
% Some thing about Colla
The reward learning curves are shown in Figure \ref{fig:reward low2}. 

\begin{figure*}[!htbp]
    \centering
\begin{subfigure}[!htbp]{0.48\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/SEnv2PS-.png}
\subcaption{Homogeneous agent in PeaRSO.}
     \end{subfigure}
       \begin{subfigure}[!htbp]{0.48\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/Env2PS-.png}
\subcaption{Heterogeneous agent in PeaRSO.}
     \end{subfigure}
     \begin{subfigure}[!htbp]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/SEnv3PS-.png}
\caption{Homogeneous agent in PeaFSO.}
  \end{subfigure}
     \begin{subfigure}[!htbp]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/Env3PS-.png}
\caption{Heterogeneous agent in PeaFSO.}
  \end{subfigure}
\caption{Comparison of agent's performance in homogeneous and heterogeneous configurations, using PPO and SAC architectures in the low demand environment. The shaded area depicts the standard deviation of the multi-agent's performance for independent experiments using 5 different seeds.}
\label{fig:reward low2}
\end{figure*}






\begin{figure*}[!htbp]
    \centering
     \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2SACEnv2.png}
  \subcaption{SAC in PeaRSO}
  \label{fig:episode}
  \end{subfigure}
    \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2PPOEnv2.png}
  \subcaption{PPO  in PeaRSO}
 \label{fig:episode}
  \end{subfigure}
    \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2SACEnv3.png}
  \subcaption{SAC  in PeaFSO}
\label{fig:episode}
  \end{subfigure}
    \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2PPOEnv3.png}
  \subcaption{PPO in PeaFSO}
\label{fig:episode}
  \end{subfigure}
    \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2SACEnv4.png}
  \subcaption{SAC in Colla}
\label{fig:episode}
  \end{subfigure}
   \begin{subfigure}[!htbp]{0.46\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/LowP1P2PPOEnv4.png}
  \subcaption{PPO in Colla}
\label{fig:episode}
  \end{subfigure}
\caption{Low Demand Reward of heterogeneous agent's performance refers to the policy mean reward that each agent receives; and the shaded area depicts the standard deviation of the heterogeneous agent's performance for independent experiments using 5 different seeds. Training is automatically terminated when convergence is achieved, as described in the text.}
\label{fig:factory-retailer-reward-low23}
\end{figure*}











